O2D2: Out-Of-Distribution Detector to Capture Undecidable Trials in Authorship Verification

The PAN 2021 authorship verification (AV) challenge is part of a three-year strategy, moving from a cross-topic/closed-set AV task to a cross-topic/open-set AV task over a collection of fanfiction texts. In this work, we present a novel hybrid neural-probabilistic framework that is designed to tackle the challenges of the 2021 task. Our system is based on our 2020 winning submission, with updates to significantly reduce sensitivities to topical variations and to further improve the system's calibration by means of an uncertainty-adaptation layer. Our framework additionally includes an out-of-distribution detector (O2D2) for defining non-responses. Our proposed system outperformed all other systems that participated in the PAN 2021 AV task.

==> sections/history.tex <==
\section{Stylometry: A Journey from Descriptive Statistics to 
Deep Representation Learning}

%========================
% Introduction of history
%========================
For long years, stylometry has been the analysis of style features that can be statistically quantified~\cite{Stamatatos2009}.
Nowadays: representation learning.
Deep Representation learning offers a powerful paradigm for mapping raw input data onto an organized embedding space.
The question arises: What makes a representation good for authorship verification? 


%========================
% Representation Learning
%========================


%=============
% Related work
%=============
\begin{itemize}
    \item BERAA: BERT fine-tuning for AA~\cite{Fabien2020}
    \item Learning Invariant Representations of Social Media Users~\cite{Andrews2019}
    \item DeepStyle: User Style Embedding for Authorship Attribution of Short Text~\cite{Hu2020}
    \item Cross-Domain AA Using Pre-trained Language Models~\cite{Barlas2020}
    \item Siamese Networks for Large-Scale AI~\cite{Saedi2019}
    \item Supressing Domain Style~\cite{Bischoff2020}
    \item Representation learning of writing style~\cite{Hay2020}
    \item Learning stylmetric representations~\cite{Ding2019}
    \item Adversrial Stylometry~\cite{Emmery2021}
    \item A Girl has a name~\cite{Mahmood2020}
    \item Obfuscation with Autoencoder~\cite{Saedi2020}
    \item A4N:~\cite{Shetty2020}
    \item Reduce and Attribute~\cite{Tschuggnall2019}
\end{itemize}



%==================================
% Paradigms in Authorship Analysis: 
%==================================
\subsection{Authorship Verification vs. Forensic Text Comparison}
% Deep Learning in Authorship Analysis?
% Ishiara papers 
% Brighting the gap
~\cite{Ishihara2020a}
